Noise Stability Optimization for Finding Flat Minima: A Hessian-based Regularization Approach

The training of over-parameterized neural networks has received much study in recent literature. An important consideration is the regularization of over-parameterized networks due to their highly nonconvex and nonlinear geometry. In this paper, we study noise injection algorithms, which can regularize the Hessian of the loss, leading to regions with flat loss surfaces. Specifically, by injecting isotropic Gaussian noise into the weight matrices of a neural network, we can obtain an approximately unbiased estimate of the trace of the Hessian. However, naively implementing the noise injection via adding noise to the weight matrices before backpropagation presents limited empirical improvements. To address this limitation, we design a two-point estimate of the Hessian penalty, which injects noise into the weight matrices along both positive and negative directions of the random noise. In particular, this two-point estimate eliminates the variance of the first-order Taylor's expansion term on the Hessian. We show a PAC-Bayes generalization bound that depends on the trace of the Hessian (and the radius of the weight space), which can be measured from data. We conduct a detailed experimental study to validate our approach and show that it can effectively regularize the Hessian and improve generalization. First, our algorithm can outperform prior approaches on sharpness-reduced training, delivering up to a 2.4% test accuracy increase for fine-tuning ResNets on six image classification datasets. Moreover, the trace of the Hessian reduces by 15.8%, and the largest eigenvalue is reduced by 9.7% with our approach. We also find that the regularization of the Hessian can be combined with weight decay and data augmentation, leading to stronger regularization. Second, our approach remains effective for improving generalization in pretraining multimodal CLIP models and chain-of-thought fine-tuning.

==> comments.tex <==

Concretely, for $i = 1, 2, \dots, n$, let $A_i\in\real^{d\times d}$ be a Gaussian random matrix, whose entries are drawn independently from an isotropic Gaussian with mean zero and variance one.

Prior work \citep{gunasekar2017implicit,li2018algorithmic} has shown that the loss surface of $\hat L(W)$ may have spurious solutions whose empirical risk is zero, but differ from the true solution (even after rotation).

Below, we argue that among all minimizers such that $\hat{L}(W) \le \epsilon$,
$U^{\star}$ incurs the lowest Hessian trace among all $d$ by $d$ matrices.









By contrast, we design a modified noise injection scheme, which works very well through a comprehensive empirical analysis, with a detailed theoretical analysis.

The next question is how this works and whether this adds utility to directly minimizing the function itself.
A naive way to instantiate this idea is to add noise to the neural network's weight before computing its gradient.
This type of noise injection has been studied before (which should not be confused with injecting label noise \citep{muller2019does,damian2021label}).
For example, a layer-wise regularization considering the different layer weight scaling performs better than this noise injection method \citep{}.

In our empirical analysis, we also observe that the naive way of perturbing the weight matrices before running SGD does not work well and only introduces marginal benefit on top of the SGD algorithm.
By contrast, we design a modified noise injection scheme, which works very well through a comprehensive empirical analysis, with a detailed theoretical analysis.







neural network training is by adding the noise perturbation to the weights before computing the gradient in SGD. However, we observe that this noise injection does not provide significant gains over SGD in our experiments of  .

One insight from our empirical analysis is that examining the min-averaging formulation can lead to algorithms that perform comparably with SAM empirically.
Thus, we believe this offers a new perspective to the existing literature, which may be worth further investigation in future work.

